On the Detection of Disinformation Campaign Activity with Network Analysis

Online manipulation of information has become more prevalent in recent years as state-sponsored disinformation campaigns seek to influence and polarize political topics through massive coordinated efforts. In the process, these efforts leave behind artifacts, which researchers have leveraged to analyze the tactics employed by disinformation campaigns after they are taken down. Coordination network analysis has proven helpful for learning about how disinformation campaigns operate; however, the usefulness of these forensic tools as a detection mechanism is still an open question. In this paper, we explore the use of coordination network analysis to generate features for distinguishing the activity of a disinformation campaign from legitimate Twitter activity. Doing so would provide more evidence to human analysts as they consider takedowns. We create a time series of daily coordination networks for both Twitter disinformation campaigns and legitimate Twitter communities, and train a binary classifier based on statistical features extracted from these networks. Our results show that the classifier can predict future coordinated activity of known disinformation campaigns with high accuracy (F1 = 0.98). On the more challenging task of out-of-distribution activity classification, the performance drops yet is still promising (F1 = 0.71), mainly due to an increase in the false positive rate. By doing this analysis, we show that while coordination patterns could be useful for providing evidence of disinformation activity, further investigation is needed to improve upon this method before deployment at scale.

==> background.tex <==
% \section{Data-Driven Disinformation}
\section{Data-Driven Strategic Information Operation Detection}
\label{sec:background}





\begin{comment}




background points 

Disinformation and SIO
	Discussion on what misinformation, disinformation, and SIO are.
	Discuss the flow of SIO research and where our paper lies. 
		Collect probable SIO community accounts
		Look for Coordination tactics ← Our works lies here
		Analyze coordination results and possible intent/message pushed by community
SIO detection vs bot detection problem


possible reference for here or for dataset
https://repository.wellesley.edu/cgi/viewcontent.cgi?article=1008&context=computersciencefaculty
\end{comment}


Bad actors have exploited the open nature of social media sites as a way to share disinformation with minimal effort. \textbf{Unlike {\it misinformation}, which refers to the spread of inaccurate news without ill-intent, {\it disinformation} seeks to deliberately spread misleading or inaccurate news for deception and manipulation of a narrative.} As Starbird et al. discuss, bad actors have leveraged social media disinformation as a conduit of manipulation to reach and deceive millions of people in the online world as part of their Strategic Information Operations (SIO) campaigns~\cite{starbird2019disinformation}. Many examples of these campaigns have been discovered over the past decade. Some of these can be attributed to state-sponsored manipulation~\cite{bovet2019influence}. Others, however, target specific demonstrations (e.g., \#BlackLivesMatter~\cite{arif2018acting}, \#WhiteHelmets~\cite{wilson2020cross}) and try to masquerade as grassroots movements (i.e., astroturfing) to appear more genuine to other online users. 
We used the term SIO throughout this paper to broadly refer to any coordinated effort to spread inaccurate information and influence public opinion, including specific disinformation efforts such as astroturfing.




\begin{figure}
	\vspace{-0.1in}
	\subfigure[Coordinated Tweet Activity]{
		\includegraphics[width=0.9\columnwidth]{figs/sotu_activity.pdf}
		\label{fig:sotu-activity}
	}%

	\subfigure[Coordination Networks]{
		\includegraphics[width=\columnwidth]{figs/sotu_network.pdf}
		\label{fig:sotu-network}
	}
	\caption{\newtext{Our work focuses in this paper is distinguishing coordinated disinformation activity against other activity found on Twitter. Unlike bot detection, which classifying a single node in the networks above, coordinated activity detection looks at how accounts interact with each other to push a message in a coordinated manner.}\lvnote{Setting aside politics, does this caption imply that SOTU was coordinated disinfo? lol. Also, should we come back to this later on when we talk about classification ?}}
	\label{fig:sotu}
\end{figure}

\newtext{


\subsection{Bot Detection}
Bot detection is an important task to hinder social media platform manipulation. We now highlight certain limitations of current bot detection mechanisms to help motivate our approach to the related problem of coordinated activity detection. While the bot detection problem has been widely studied for the past decade~\cite{martino2020survey,cresci2020decade} \penote{cite any more?}, the evolving nature of social media sites has made bot detection less promising. Two major factors contribute to this issue. First, bot detection is a classification problem that seeks to determine if an account is human or a robot, without considering intent, by measuring possible automation metrics (e.g., time of tweet, creation time, generated usernames). While these metrics were enough to detect fake accounts in the earlier years, bad actors have become more sophisticated,. At the same time, regular users have also gained the ability to have more automated control over their account (e.g., time-released tweets, API access, multi-person control). Since bot detection focuses on automation, these factors have caused promising bot detection tools, such as Botometer~\cite{varol2017online}, to have a high false-positive rate when tested against normal users~\cite{rauchfleisch2020false}.

The second issue faced by current bot detection methods is the focus of classifying a singular fake account. With the emergence of orchestrated efforts, such as SIO campaigns, platform manipulation has been done by creating multiple sock puppet accounts, all of which boost the signal of their messages to seem more authentic for regular users. Since these sock puppet accounts coordinate together, bot detection does not leverage the similarities between accounts to classify a campaign.


\subsection{Coordinated Activity Detection}

Rather than focusing on single accounts, coordinated activity detection requires looking into behavior across accounts since SIO campaigns tend to rely on many accounts to push their message (Figure~\ref{fig:sotu}). Many researchers already leverage coordination network graphs as a way to do a {\it postmortem} forensic analysis of SIO campaigns that have been taken down \lvnote{[cite a ton of papers].} While these coordination networks have helped in understanding how SIO campaigns operate, it is still unclear if networks produced by coordination networks could be used as evidence to detect SIO activity before the campaign is found and taken down. 

An ideal SIO detection tool would flag a network of accounts that are spreading disinformation in a coordinated fashion. This problem can be broken down into two main subtasks: identifying suspicious communities by looking at coordination patterns amongst the members and identifying the intent of the messages the accounts promote. The intent is usually determined by human analysts that understand the context of how/when the messages were shared. While some researchers have inferred the intent of a campaign based on offline data (e.g., email leakages~\cite{king2017chinese}, court filings~\cite{keller2017manipulate}), such data sources are rarely available, making intent identification an open problem. We do not focus on predicting the intent of disinformation activity and leave it to the analysis of the intelligence community. In this paper, instead of SIO (or bot) detection, we focus on coordinated activity detection as a way to provide {\it evidence} on whether the activity of a group of accounts appears to be SIO-like. This evidence could then help human analysts determine the authenticity of said group and lower the time to takedown SIO campaigns. 

To arrive at this goal, we conduct a large-scale analysis of the coordination patterns found in Twitter SIO campaigns using tweets from Twitter's Information Operations Election Integrity report~\cite{twitterElectionHub} as well as tweets from political and non-political Twitter communities that engage in legitimate coordination. 




% In fact,  These works include looking at the similar content/timing of post of the tweets the accounts share. While this form of  forensic {\it post-mortem} analysis has been valuable to understanding how SIO campaigns operate, it is unclear whether such form of coordinated activity could be use to detect SIO campaigns before the the information diffused throughout social media. To that end, our work focuses on using coordinated activity as a form of detection mechanism for SIO communities.

% Currently, by the time an SIO campaign have been taken down, the messages of the campaign may already have had influence real people that have engaged with the posts of the accounts. Unfortunately, takedowns of SIO campaigns could take months or years, which leaves a long time for inauthentic content to be shared. As such, it is important to have a rapid detection mechanism for SIO campaign. One prominent feature that is used for postmortem analysis is to see how much coordination occurs amongst accounts belonging to the SIO campaign. While measuring coordination via network analysis has been used for post mortem analysis, it is still unclear if coordination via network analysis could be used for fast detection of SIO campaigns. Note SIO cam



}





\oldtext{
\subsection{Operating a Disinformation Campaign}


\lvnote{We might get rid of this whole sections and replace it with coordianted activity}
Disinformation campaigns can be carried out by multiple state and non-state operators. The goal of these campaigns is to manipulate a narrative and deliberately share misleading or confusing information to the broader public while staying camouflaged. To reach this goal, disinformation campaigns have successfully exploited the open nature of social media sites. For example, previous research discovered how Russia's Internet Research Agency (IRA) and Iran's state-sponsored apparatus launched social media disinformation campaigns attacking the United State's presidential election in 2016~\cite{russia2016,iran2018}.


% There are various approaches to operating a disinformation campaign. The most simplistic is to create a single account and start sharing false information. This, however, does not maximize the goal of reaching the broader audience the campaign wishes to deceive. Therefore, 
Disinformation campaigns are usually composed of hundreds to thousands of accounts. As explained by Keller et al.~\cite{keller2020political}, the operation of these campaigns can be roughly described by the principal-agent theory~\cite{miller2005political,ross1973economic}, where the principal (campaign operator) conducts the agents (user accounts) to perform some task (spread false information). In the principal-agent problem, an issue arises when agents act for their own best interest, which is against the priorities of the principal. While carrying out the task of spreading disinformation, the agents are capable of making a decision that may hurt the camouflaging goal of the campaign operator by making use of automation. As such, disinformation campaigns need to balance the natural duality that exists between actively spreading misleading content and camouflaging their efforts to avoid detection. If the agents are purely automated, then it is easier for more agents to spread misleading messages. However, detecting the activity becomes a more manageable task due to the behavioral artifacts automation may leave behind (e.g., bulk account creation, temporal patterns, account inauthenticity)~\cite{liu2015exploiting,fu2017robust,cao2012aiding}. Conversely, if human agents controlled the accounts, then more resources are needed, and fewer accounts may be available to spread the message. However, even though there are fewer accounts, they have a higher chance of being more authentic to the human users the campaign wishes to manipulate, thereby camouflaging the disinformation campaign. \lvnote{Do we still need this paragraph? It's a lot of exposition. While I like it, we may need to get rid of it for space purposes.}


Regardless of the type of agents (automated or human), the accounts that are part of the disinformation campaign may need to coordinate amongst themselves to push the message they wish to manipulate. This is seen by looking at the historical activity of the accounts that post similar messages at around the same time. It is this type of coordination that researchers have tried to exploit as a way to detect if a disinformation campaign is being executed~\cite{ratkiewicz2011truthy,ratkiewicz2011detecting,keller2017manipulate}.


\lvnote{This should be its own subsection. That we we clearly state what are goal is early in the paper}
In this work, we set out to analyze coordination found in Twitter communities with the goal of characterizing the issues coordination-based SIO detection tools may have. For an SIO detection tool, the ultimate goal would be to flag a user community (i.e., a network of accounts) that has spread disinformation in a coordinated fashion. This problem can be broken down into two main subtasks: identifying suspicious communities by looking at coordination patterns amongst the members and identifying the intent of the messages the accounts promote. The intent is usually determined by human analysts that understand the context of how/when the messages were shared. While some researchers have inferred the intent of a campaign based on offline data (e.g., email leakages~\cite{king2017chinese}, court filings~\cite{keller2017manipulate}), such data sources are rarely available, making intent identification an open problem. We do not focus on the intent of disinformation and leave it to the analysis of the intelligence community. 
%Instead, we analyze coordination amongst community members, which is a more measurable effort.
Instead, to arrive at our goal of carefully assessing coordination-based SIO classifiers, we conduct a large-scale analysis of the coordination patterns found in Twitter SIO campaigns using tweets from Twitter's Information Operations Election Integrity report~\cite{twitterElectionHub} as well as tweets from political and non-political Twitter communities that engage in legitimate coordination. 
}

==> dataset.tex <==






==> eval_ccs.tex <==



\section{Analysis}
\label{sec:analysis:results}

\lvnote{Honestly, this section only needs an update to the numbers and to mention the rolling time windown}

\begin{figure*}[th]

	\subfigure[Iran  $\rightarrow$  Geopolitics]{
		\includegraphics[width=0.235\textwidth]{figs/iran_activity.pdf}
		\label{fig:iran}}
	\subfigure[Venezuela (commercial) $\rightarrow$  Venezuela]{
		\includegraphics[width=0.235\textwidth]{figs/venezuela_activity.pdf}
		\label{fig:venezuela}}
	\subfigure[US Congress]{
		\includegraphics[width=0.235\textwidth]{figs/congress_activity.pdf}
		\label{fig:congress}}
	\subfigure[Academics]{
		\includegraphics[width=0.235\textwidth]{figs/academics_activity.pdf}
		\label{fig:academics}}
	\caption{Examples of coordination activity for four communities (two disinformation campaigns and two of the manually collected baselines). Each community appears to have different behavior characteristics such as high levels of co-tweeting (Venezuela (commercial) or diversity in employed coordination patterns (Iran). A variety of coordination patterns can be seen more extensively in political communities (e.g., US Congress) than non-political (Academics), but both types of baselines show increasing amounts of coordinated activity over time.}
	\label{fig:activity}
\end{figure*}

To answer the research questions posed in Section~\ref{sec:meth}, we conduct a series of empirical studies. First, we qualitatively characterize how coordination changes in communities. Then, to answer \textit{RQ1}, we measure the ability of our binary classifier to correctly identify the daily/weekly coordinated tweet activity by the considered Twitter SIO campaigns and baseline Twitter communities. We interpret the trained models by visualizing the coordination feature vectors using t-SNE \cite{maaten2008visualizing} and discuss feature importance using SHAP plots \cite{NIPS2017_7062}. We address \textit{RQ2} by presenting a case study on COVID-19 Twitter activity collected from members of the UK Parliament and the US Congress. Our case study shows how a massive global event has lead to an increase in SIO-like Twitter coordination from political communities, which in turn negatively impacts the ability of classifiers to identify SIO campaigns. 

\begin{figure*}
	\subfigure[Daily coordination activity]{
		\includegraphics[width=0.45\textwidth]{figs/tsne_daily_1_min_threshold.pdf}}%
	\subfigure[Weekly coordination activity\label{fig:tsne_weekly}]{
		\includegraphics[width=0.45\textwidth]{figs/tsne_weekly_1_min_threshold.pdf}
	}
	\caption{Visualizing t-SNE plots of the training set coordination feature vectors for SIO campaigns and baselines (political and non-political) shows that the feature vectors generally appear to be separable at (a) daily aggregation and even more so with weekly aggregation (b). However, on days when a community is reacting to specific events (e.g., US SOTU addresses, UK general election), coordination from political communities blends in with SIO-like activity. This can be clearly seen by looking at baseline events (indicated by stars) that are near the vicinity of SIO activity, and by seeing that in b) the various weeks of heavy political activity (e.g., US SOTU addresses) become even more dissimilar from other baseline activity.}
	\label{fig:tsne}
\end{figure*}


\subsection{Characterization of Coordination}
\label{section:analysis:high-level-char}

\subsubsection{Setup}
Before we analyze the guiding questions mentioned in Section~\ref{sec:meth}, we first do a high-level characterization of the coordination found in both the SIO campaigns as well as our baselines. In Figure~\ref{fig:activity}, we show examples of the coordination patterns exhibited by some of the SIO campaigns and baselines. We generated the coordination networks for each pattern discussed in Section~\ref{sec:features} using daily aggregation with a 1-minute time threshold. We then counted how many accounts participated in each coordination pattern within their respective communities in a given day (i.e., the number of nodes in the coordination network). Note that each column represents the coordination patterns for one campaign, and the y-axis of the columns are different. Due to space limitations, we show the rest of the coordination patterns in Appendix~\ref{appendix:mapping}.
Furthermore, to check how separable SIO and non-SIO coordination activity is, we visualize t-SNE plots of the training set feature vectors corresponding to daily/ weekly aggregation at a 1-minute time threshold in Figure~\ref{fig:tsne}. We found that PCA \cite{tipping1999probabilistic} was unable to produce an interpretable representation of the variety of coordination activity in our data; t-SNE is a more expressive dimensionality reduction tool for visualizing high dimensional datain a 2-D plane. The features can be colored by class label to help reveal similarities across distinct classes in the dataset.


\subsubsection{Key Results}
We find that the usage of each type of coordination pattern differs from one community to the next. From Figure~\ref{fig:activity}, we can see that coordination in SIO campaigns appear to be more orchestrated. For example, in the Iranian campaign (Figure~\ref{fig:iran}), the community appears to make use of co-tweeting (yellow) in late 2015 but then stops soon after. They then switch to coordinating by using low amounts of retweeting (red) and high amounts of co-retweeting (green) for the majority of 2017. Conversely, coordination for the Venezuela (commercial) campaign (Figure~\ref{fig:venezuela}) posted the same message from each account (co-tweeting). These SIO campaigns show relatively constant coordinated activity, whereas other SIO campaigns (Appendix~\ref{appendix:mapping}) show different bursty behaviors (i.e., intermittent levels of high activity and little to no activity). 
% \lvnote{I don't know if we should add this last sentence. It feels like we would be going into temporal dependencies} 
% \penote{Maybe remind the reader here that we already stated accounting for temporal dependencies is not addressed in our study?}

For the baseline communities, we can see that retweeting is the most used coordination pattern. This is not surprising as retweeting is one of the most common actions that a user can take on Twitter as it only takes one click. Additionally, accounts within a community may desire to signal boost each other by retweeting if they share similar goals (e.g., legislative or academic). The amount of coordination also varies for the baselines, with political communities (the UK Parliament and the US Congress) showing more coordination than our non-political communities (Random and Academics). Finally, we note that while co-tweeting patterns are minimal in all of the baseline communities, some SIO campaigns rarely employ co-tweeting, thereby preventing the use of only co-tweeting metrics as a simple rule for identifying SIO activity. 

Additionally, in Figure~\ref{fig:tsne}, we observe that the feature vectors of coordinated activity appear to cluster into SIO, political, and non-political for both daily and weekly coordination patterns. We first note that days and weeks of low coordination activity are present in the training sets for both SIO campaigns and the baselines. These low activity days manifest in the t-SNE plots as tight, isolated clusters where data points from all three clusters overlap. 
% They do not affect the classifier while validating on the held-out data, however, since we validate on the last 15\% of days/weeks of campaigns/baseline communities during which there are rarely lulls in coordination activity. 
Another noticeable aspect is that there are several isolated days/weeks of political activity (green) that are spread through the SIO activity. Many of these days turn out to correspond to events of note such as the 2018 and 2019 US State of the Union (SOTU) addresses (we investigate further in Section~\ref{sec:analysis:misclass}). The proximity of these political days to SIO coordination feature vectors shows that during community events, some baselines appear to have SIO-like activity patterns. Finally, we find that increasing the temporal aggregation from daily to weekly greatly increases the separation between non-political and SIO coordination. While certain amounts of political coordination now resemble neither non-political nor SIO activity (2017 UK general elections in Figure~\ref{fig:tsne_weekly}), other instances (2018 and 2019 US SOTU) appear even more strongly to be SIO activity.


\subsubsection{Takeaways}
As expected, coordination appears to be more prevalent and orchestrated in SIO campaigns than in the baseline communities. However, the type of coordination, as well as the behavior based on it, differs for each campaign and community. These variations can make it hard for detection mechanisms to learn generalizable patterns to detect SIO-like activity, which is worsened by the observation that the amount of coordination tends to increase over time. Moreover, the activity from days where a legitimate community reacts to a specific event appears to closely resemble SIO-like coordination patterns. 

\subsection{RQ1: Coordination Activity Classification}
\label{sec:analysis:classification}

%  RQ1: Can we train a classifier to distinguish daily/weekly activity of  Twitter communities vs. Twitter SIO using network analysis features
% 1.(all pre-2020 data). Let's do some intuition building with t-SNE plots
% 2. Quantitative results: F1 / FPR / Feature importance
% 3. Qualitative results: What events were captured by the errors made by the classifier?
% Discussion: daily vs. weekly, events occuring on days/week scale



\begin{figure}
\vspace{-0.1in}
\subfigure[P-R Curve (daily / 1-minute)]{
	\includegraphics[width=0.9\columnwidth]{figs/daily_1_min_threshold_pr_curve_ppv.pdf}
}
\subfigure[P-R Curve (weekly / 1-minute)]{
	\includegraphics[width=0.9\columnwidth]{figs/weekly_1_min_threshold_pr_curve_ppv.pdf}
}
\vspace{-0.1in}
\caption{P-R curves for the daily / 1-minute and weekly / 1-minute models that had a PR-AUC score closest to the mean PR-AUC across 10 folds. F1 scores at P = 0.975 are marked by stars. a) We found that daily coordination aggregation performs better than weekly aggregation at identifying political community activity, but the recall at sufficiently high precision allows nearly 20\% of SIO activity to pass by undetected (UK Parliament R = 0.83, US Congress R = 0.78).  b) Weekly aggregation is best for non-political communities, with our classifier obtaining F1 (P-Threshold) scores of 0.99 for both non-political baselines. The sharp drop in F1 (P-Threshold) score for the UK Parliament and US Congress models between daily/weekly shows that relaxing the strict false positive requirement is necessary to detect SIO activity using larger temporal aggregation; however, high false positive rates severely degrade the usability of automated detection tools.}
\vspace{-0.1in}

	\label{fig:pr_curves}
\end{figure}


\begin{table}[]
\begin{center}
\begin{tabular}{@{}c|c|cc@{}}
\toprule
                          F1  ($\uparrow$)    & Activity        & Political & Non-political \\ \midrule
\parbox[t]{0mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{Voting}}}     & Daily / 1-min   & \textbf{0.91 (0.89, 0.92)}     & 0.94 (0.92, 0.97)         \\
                                                    & Daily / 5-min   & 0.86 (0.84, 0.88)      & 0.92 (0.88, 0.96)         \\
                                                    & Daily / 10-min  & 0.83 (0.81, 0.86)      & 0.91 (0.86, 0.95)          \\ \cmidrule(l){2-4} 
                                                    & Weekly  / 1-min & 0.89 (0.87, 0.91)     & 0.97 (0.95, 0.98)         \\
                                                    & Weekly / 5-min  & 0.83 (0.81, 0.85)     & 0.94  (0.91, 0.96)        \\
                                                    & Weekly / 10-min & 0.80 (0.79, 0.82)      & 0.94  (0.91, 0.97)        \\ \midrule
\parbox[t]{0mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{P-Threshold}}}   & Daily / 1-min   & 0.83 (0.76, 0.90)    & 0.94 (0.91, 0.98)          \\
\multicolumn{1}{l|}{}                               & Daily / 5-min   & 0.62 (0.52, 0.72)      & 0.86  (0.75, 0.97)        \\
\multicolumn{1}{l|}{}                               & Daily / 10-min  & 0.52 (0.40, 0.65)      & 0.91 (0.85, 0.97)          \\ \cmidrule(l){2-4} 
\multicolumn{1}{l|}{}                               & Weekly / 1-min  & 0.66 (0.55, 0.78)      & \textbf{0.99 (0.99, 1.0)}        \\
\multicolumn{1}{l|}{}                               & Weekly / 5-min  & 0.45 (0.31, 0.59)      & 0.98 (0.97, 0.99)         \\
\multicolumn{1}{l|}{}                               & Weekly / 10-min & 0.42 (0.28, 0.55)     & 0.98  (0.97, 0.99)       
\end{tabular}
\end{center}
\vspace{0.1in}
\caption{10-fold CV F1 scores. F1 scores are averaged across 10 folds with 95\% (upper, lower) confidence intervals around the mean estimate shown. F1 (P-Threshold) scores are evaluated at the threshold corresponding to P = 0.975 along the P-R curve. \label{tbl:F1}}

\end{table}

\begin{table}[t]
\begin{center}
\begin{tabular}{l|c|c}
\toprule
 10-fold CV    & \begin{tabular}[c]{@{}c@{}}TPR / TNR\\ P-Threshold\end{tabular} & \begin{tabular}[c]{@{}c@{}}TPR / TNR\\ Voting\end{tabular} \\
 \midrule
Political (daily / 1-min)  &\textbf{0.75} / \textbf{0.98}           & \textbf{0.93}  / \textbf{0.87}                                                       \\ 
Political (daily / 5-min)  & 0.49   / 0.99            & 0.90  / 0.77                                                                                  \\ 
Political (daily / 10-min) & 0.40  / 0.99                 & 0.88 / 0.72                                                                                 
\end{tabular}
\end{center}
\caption{TPR = true positive rate (recall), TNR = true negative rate (specificity). Here, TPR measures the ability of the classifier to find all of the SIO instances. TNR measures the ability of the classifier to correctly identify coordination from the US Congress (N = 361) and the UK Parliament (N = 367). \label{tbl:tpr_tnr}}
\end{table}


\subsubsection{Setup} Using the cross-validation data splits described in Section \ref{sec:implementation}, we now train all of the binary classifiers and analyze their ability to distinguish daily/weekly coordinated activity from our SIO and non-SIO Twitter communities.
In Table~\ref{tbl:F1}, we show F1 (Voting) and F1 (P-Threshold) scores computed by averaging over the 10 cross-validation folds, political communities (UK Parliament and US Congress), and non-political communities (Academics and Random) with 95\% confidence intervals (CI) shown. For each of the 10 folds, we evaluate F1 (P-Threshold) at the threshold corresponding to P = 0.975. To select one model from the 10 folds for displaying precision-recall curves, we compute the average PR-AUC score across the 10 models and select the one whose PR-AUC score is closest to the mean. We do this rather than selecting the model that achieves the highest PR-AUC score across the 10 folds since we observed that the best PR-AUC score consistently fell outside of the 95\% CI of the mean, and is likely to overestimate the results. The daily / 1-minute precision-recall curves are shown in Figure~\ref{fig:pr_curves}, with the remainder of the curves shown in Appendix~\ref{appendix:mapping}. For a more fine-grained examination of the performances, sensitivity vs. specificity for the daily / 1-minute models is shown in Table~\ref{tbl:tpr_tnr}.


\subsubsection{Key Results}
The daily / 1-minute models all attain F1 (Voting) scores greater than or equal to 0.91, and when increasing aggregation to weekly / 1-minute, the F1 (Voting) scores for non-political communities increases to 0.97. Strikingly, the F1 (P-Threshold) scores at weekly / 1-minute for non-political communities reach 0.99. Conversely, when moving from daily to weekly, the classifier either has low recall when achieving the threshold on false positives for political communities (F1 (P-Threshold) = 0.66) or sacrifices precision to maintain a high F1 score (F1 (Voting) = 0.89). 

By requiring P = 0.975, the specificity for the political communities at daily / 1-minute is acceptable (TNR = 0.98) but the trade-off is a lower recall (R = 0.75). On the other hand, using voting to decide labels achieves a more balanced trade-off of specificity (TNR = 0.87) and recall (R = 0.93), but a TNR of 0.87 does not reflect our desire for a sufficiently low rate of false positives. 


\subsubsection{Takeaways}


We conclude that by adequately tuning the decision threshold and using weekly aggregation, the RF classifier can achieve near-perfect separation of non-political coordination from SIO coordination. However, the same cannot be said about political communities. While the F1 scores (both Voting and P-Threshold) for the political communities appear high, there is still a false positive problem when achieving desirable recall levels. More broadly, these results show that disinformation detection based on network analysis must balance effectiveness for usability. With a loose restriction on the number of allowable false positives, a classifier can identify almost all of the SIO activity, but such a system would be deemed impractical as it would flag a high amount of benign activity.  Therefore, our response to RQ1 is that a classifier using only network analysis features is \textit{unable} to distinguish daily/weekly activity as SIO or non-SIO at desirable levels for \textit{all} Twitter communities.

We noticed that many of the errors causing the false positives surrounded days/weeks, which contained significant political events (see Section \ref{sec:analysis:misclass}). We also note that increasing the time thresholds to 5 and 10 minutes tended to reduce model performance, suggesting that the added coordination captured by higher time thresholds has the effect of further blurring the line between legitimate coordination found in Twitter communities and SIO activity.  

To further probe the classifier's decision-making process, we produced a SHAP summary plot of RF feature importances (Figure \ref{fig:shapley}). As our focus is on assessing the broad use of network analysis features for our detection task, we do not analyze the features in further detail by examining e.g., partial dependence plots or multicollinearity in this study. The classifier mostly relies on various statistics of the retweet network to separate SIO and non-SIO data. 
%We often found that daily or weekly political coordination containing a variety of coordination types tended to be misclassified, but days or weeks with high amounts of retweets tended to be correctly classified \penote{Is this fair?}\lvnote{I don't think we can prove this... at least right now}.
 A high average node degree in the retweet network is a main indicator of SIO activity, however. Other important coordination features that strongly indicate similarity to SIO activity include the number of nodes in the co-tweet network, as well as the average size of connected components of the co-url and co-mention networks. Co-tweeting rarely appears in the non-SIO training data, causing the classifier to label almost all data points containing any amount of co-tweeting as SIO. Overall, stronger connectivity amongst nodes increases the likelihood that the classifier labels the activity as SIO.



\begin{figure}[t]
\includegraphics[width=0.9\columnwidth]{figs/shapley.pdf}
\vspace{-0.2in}
\caption{SHAP feature importance (top to bottom). Retweet network activity metrics are most informative for the classifier to separate SIO campaigns and baseline communities.}
	\label{fig:shapley}
\end{figure}


\subsection{RQ1: Examples of Misclassification}
\label{sec:analysis:misclass}


\begin{figure}
	\vspace{-0.1in}
	\subfigure[Coordinated Tweet Activity]{
		\includegraphics[width=0.9\columnwidth]{figs/sotu_activity.pdf}
		\label{fig:sotu-activity}
	}%

	\subfigure[Coordination Networks]{
		\includegraphics[width=\columnwidth]{figs/sotu_network.pdf}
		\label{fig:sotu-network}
	}
	\caption{Example of a day in which the US Congress Twitter activity was misclassified as resembling SIO-like coordination patterns. The misclassification is mostly attributed to the US Congress reacting to the 2020 US State of the Union address (note the UTC time). We show the tweet count for tweets that were part of the coordination networks.}
	\label{fig:sotu}
\end{figure}


\subsubsection{Setup} We now turn our attention to understanding why coordination activity of legitimate communities can get misclassified as SIO activity, due to the emphasis we place on minimizing false positives. To do that, we look at the days that were consistently misclassified by the daily / 1-minute models across each of the 10 folds in cross-validation. More concretely, we only consider days in this analysis if they were misclassified across \textit{all} CV folds. We found 0 days from Academics, 9 days for Random, 16 days for the US Congress, and 13 days for the UK Parliament. We then extract all information from the tweets that were used to generate the coordination network for that given day. Finally, we manually looked at both the tweets that caused the misclassification to occur as well as the news for that specific date that may have affected the coordination patterns of the community. 

\subsubsection{Key Results} Unsurprisingly, the models that validated their ability to classify non-SIO activity on \textit{non-political} communities did not make many misclassifications.  Mainly, we noticed that the coordination networks based on co-url and co-hashtag appeared to be more active while other networks (e.g., retweet network) had minimal (if any) activity. For the dates that were misclassified, we could not determine any specific event that caused the error. As discussed in Section \ref{sec:analysis:classification}, by increasing the temporal aggregation to weekly / 1-minute, the RF can reduce misclassifications to nearly 0.

Conversely, for the political baselines, we noticed that the misclassifications occur when the community is reacting to a specific community event. For example, in the US Congress dataset, we saw that the US Congress Twitter activity surrounding the impeachment hearings of President Donald Trump was mostly misclassified as having SIO-like coordination patterns. These misclassified dates include the announcement of a formal impeachment inquiry~\cite{impeachmentFormal}, many days during the testimonial hearings~\cite{impeachmentWeek}, and the House vote to pass the Articles of Impeachment~\cite{impeachmentVote}. Furthermore, as Figure~\ref{fig:tsne} demonstrates, the coordination pattern surrounding events like the 2018 and 2019 SOTU address appears similar to SIO coordination. Indeed, the 2020 SOTU was also consistently misclassified. In Figure~\ref{fig:sotu}, we show the coordination activity as well as the generated networks of US Congress during the SOTU address of 2020. Note that highly coordinated tweet activity occurs at the same time as the event is on the air.\footnote{While misclassified day may be cause due to event, other days appear to be misclassified due to constant tweet activity throughout the whole day.} The UK Parliament was no different in regards to misclassification. Many days misclassified included Prime Minister Boris Johnson becoming the leader of the Conservative Party, updates on the UK withdrawing from the European Union (i.e., Brexit), or debates regarding the general elections for the UK.

\subsubsection{Takeaways} The findings above may have profound implications beyond the classification of coordinated community activity. The coordination networks are subgraphs of the monolithic coordination network generated on the entire activity of the whole community. SIO community detection systems are likely to have many false positives if they are based on monolithic networks that naively aggregate over long time periods since legitimate communities would appear as highly coordinated, even though the coordination may only occur around community events, which are expected to be common occurrences across Twitter. Information on those events, however, is lost since the monolithic network ignores the temporal nature of the activity.

\begin{table}[th] 
\begin{center}
\begin{tabular}{@{}l|cc@{}}
\toprule
 March 1, 2020\textemdash                           & \begin{tabular}[c]{@{}c@{}}TNR\\  P-Threshold\end{tabular} & \begin{tabular}[c]{@{}c@{}}TNR\\  Voting\end{tabular} \\ \midrule
UK Parliament (daily / 1-min)   &  0.68                                                                    & \textbf{0.45}                                                                \\
UK Parliament (daily / 5-min)           & \textbf{0.8}                                                                     & 0.31                                                                \\
UK Parliament (daily / 10-min)          & 0.7                                                                  & 0.26                                                               \\ \midrule
US Congress (daily / 1-min)     & 0.92                                                                  & \textbf{0.64}                                                                \\
US Congress (daily / 5-min)          &  \textbf{0.97}                                                                    & 0.42                                                                \\
US Congress (daily / 10-min)         & 0.79                                                                    & 0.45   \\     
\end{tabular}
\end{center}
    \caption{Classifier specificity/TNR on post-COVID-19 Twitter activity for UK Parliament (N = 32)  and US Congress (N = 51). TNR = true negative rate. \label{tbl:COVID}}
\vspace{-0.1in}

\end{table}


\subsection{RQ2: Case Study---Political Coordination During the COVID-19 Pandemic}
\label{sec:analysis:covid}
% How does UK Parliament’s/Congress' FPR/F1 scores change if we include up to April 1 2020 in the validation set? In the train set?
% Other ways to characterize to what extent coordination activity has changed due to COVID-19 for Parliament and Congress? Pearson correlation?

\subsubsection{Setup}
% \penote{Cite a news article for the date?}
While conducting this study, we observed a shift in the coordination patterns of the political communities around the time the COVID-19 pandemic began to impact western countries (late February 2020). This enabled us to conduct a unique case study to test the generalization ability of our trained models in a novel environment; that of a global event that has required governments to take drastic actions and assert varying levels of influence over their populations. \textit{Arguably, this is when SIO campaigns could be most damaging, making detection critical.} We test the daily UK Parliament and US Congress models against UK Parliament and US Congress Twitter activity collected via the Twitter API after \mbox{2020-3-1}. We average the specificity over the 10 CV models, using both the P = 0.975 decision thresholds as well as voting, and compare the specificity (Table~\ref{tbl:COVID}) to the reported specificity from the pre-COVID-19 validation sets (Table~\ref{tbl:tpr_tnr}).  The case study included 32 days for the UK Parliament  and 54 days for the US Congress baselines.


\subsubsection{Key Results} When using voting, the ability of the daily / 1-minute model to classify UK Parliament activity after March 1 is reduced significantly (TNR = 0.45) with better results for classifying US Congress activity (TNR = 0.64). This is a stark contrast to the cross-validation specificity scores reported earlier; the best pre-COVID-19 average specificities for political communities are 0.98 (P-Threshold) and 0.87 (Voting) using daily / 1-minute, and the best post-COVID-19 average specificities are 0.88 (P-Threshold) daily / 5-minute and 0.54 (Voting) daily / 1-minute. \textit{Effectively, the voting-based classifier, which achieves the best pre-COVID-19 recall of 0.93, has its specificity decrease by 33 percentage points ($0.87 \rightarrow 0.54$) post-COVID-19}. The recall for the daily / 5-minute model pre-COVID-19 is just 0.49 (P-Threshold). We can attribute the low scores to the increases in political coordination in March 2020. We visualize this by showing the t-SNE plot of the daily feature vectors for political communities during the COVID-19 pandemic along with the SIO and political community training data (Figure \ref{fig:COVID}). Almost all of the days after 2020-3-1 are near other days of substantial political coordination, such as the SOTU addresses. If it is allowable for the model to miss 25\% of SIO activity while maintaining low false positives, the daily / 1-minute model (P-Threshold) can identify 80\% of legitimate political coordination during the COVID-19 pandemic. However, this low recall score is likely ineffective for a practical and scalable SIO detection system. 

\subsubsection{Takeaways} The increase in political coordination exhibited by the US Congress and even more so by the UK Parliament due to the COVID-19 pandemic is reflected by a corresponding sharp decrease in our trained models ability to identify non-SIO coordination. By increasing the detection threshold, the classifier can somewhat identify political activity as non-SIO, but a broader discussion about an acceptable recall for detecting SIO activity must be held. Note that in our training dataset, we have slightly more positive labels than negative labels (4:3 ratio), which implies that maintaining the P = 0.975 with a more imbalanced dataset where the non-SIO labels dominate would lead to even lower recall scores. Hence, in response to RQ2, we show that the extent at which such a global event affects our network analysis-based classifier highlights that bad actors that try to take advantage of time periods such as these to deploy an SIO campaign are less likely to be detected.


\begin{figure}
\includegraphics[width=\columnwidth]{figs/tsne_daily_1_min_threshold_covid.pdf}
\vspace{-0.3in}
\caption{COVID-19 t-SNE data visualization. The unexpected surge of activity from the UK Parliament and the US Congress due to the COVID-19 pandemic makes it difficult to differentiate between SIO-like coordinated activity and the governments online discussion.
	\label{fig:COVID}}
\vspace{-0.1in}

\end{figure}

% \subsection{RQ3: Exploring Coordination Network Structure}
% \label{sec:analysis:structure}
% % Does removing weak coordination (small CCs) further improve the distinction between SIO and political communities?
%        % Show F1 / FPR after tweaking
% % Transitive coordination
%        % Show F1 / FPR after tweaking

% \iffalse
% . Filtering removes like 90% of random_walk train days . We remove close to 40% of uae_quatar_yemen, iran_geopolitics, and uaeegypt_multiple as well...
% we don't know whether its actually filler or not. That requires further analysis that goes beyond what coordination features can do. any threshold we set would have to be arbitrary
% \fi 
% % Explanation: For each of 6 coordination network types (co-tweet, co-retweet, co-url, co-mention, co-hashtag) with per-day 1-minute activity threshold, we compute these statistics and concatenate the result into a 42-dimensional vector.
%\begin{table}[t] 
%    \caption{Features used for binary classification \label{tab:features}}
%     \begin{tabular}{c|l}
%          \toprule
%      	\texttt{nodes} & Number of nodes in the coordination network \\
%      	\texttt{edges} & Number of edges  in the coordination network \\
%      	\texttt{largest\_cc} & Size of the largest connected component \\
%      	\texttt{mean\_cc} & Average size of connected components \\
%      	\texttt{std\_dev\_cc} & Std. dev. of the sizes of connected components \\
%	\texttt{mean\_deg} & Average degree of nodes  in the coordination network \\
% 	\texttt{std\_dev\_deg} & Std. dev. of node degrees in the coordination network \\
%    \end{tabular}
%    \vspace{-0.1in}
%\end{table}

% Explanation:  when holding out each Twitter community from the training set, averaged over 10 CV folds (leaving out 2 SIO campaign) 
%\begin{table*}[t] 
%\caption{10-Fold CV Average F1 score---RF Voting ($\uparrow$) \label{tab:F1}}
%\begin{center}
%     \begin{tabular}{l|c|cccc}
%          \toprule
%	Activity & All & UK Parliament & US Congress & Academics & Random \\
%      	\midrule
%		Daily / 1 min & 0.92 & \textbf{0.90} & \textbf{0.91}  & 0.95 & 0.93 \\
%		Daily / 5 min &0.89 & 0.84 & 0.87  & 0.93 & 0.91 \\
%		Daily / 10 min & 0.87 & 0.81 & 0.86  & 0.91 & 0.90 \\
%		\midrule
%		Weekly / 1 min & 0.93 & \textbf{0.90} & 0.88  & \textbf{0.97} & \textbf{0.97} \\
%		Weekly / 5 min &0.88 & 0.82 & 0.83 & 0.93 & 0.94 \\
%		Weekly / 10 min & 0.87 & 0.80 & 0.81  & 0.94 & 0.94
%    \end{tabular}
%    \vspace{-0.1in}
%\end{center}
%\end{table*}
%
%\begin{table}[]
%\caption{10-Fold CV F1 score---PPV Threshold ($\uparrow$) \penote{TODO figure out how to combine this with the other table} \label{tab:F1-PPV}}
%\begin{center}
%\begin{tabular}{@{}c|cccc@{}}
%\toprule
%                                                         & UK Parliament & US Congress   & Academics     & Random        \\ \midrule
%\begin{tabular}[c]{@{}c@{}}Daily \\ 1 min\end{tabular}   & \textbf{0.90} & 0.87          & 0.97          & 0.91          \\ \midrule
%\begin{tabular}[c]{@{}c@{}}Daily\\ 5 min\end{tabular}    & 0.59          & 0.63          & 0.97          & 0.92          \\ \midrule
%\begin{tabular}[c]{@{}c@{}}Daily \\ 10 min\end{tabular}  & 0.38          & 0.64          & 0.97          & 0.88          \\ \midrule
%\begin{tabular}[c]{@{}c@{}}Weekly \\ 1 min\end{tabular}  & 0.27          & 0.66 & \textbf{0.99} & \textbf{0.99} \\ \midrule
%\begin{tabular}[c]{@{}c@{}}Weekly \\ 5 min\end{tabular}  & 0.12          & 0.73          & 0.98          & 0.99          \\ \midrule
%\begin{tabular}[c]{@{}c@{}}Weekly \\ 10 min\end{tabular} & 0.50          & 0.11          & 0.98          & 0.97         
%\end{tabular}
%\end{center}
%\end{table}

% for certain setups e.g., weekly 1 min, our RF can learn to almost perfectly classify Academics/Random data, suggesting that our slight label imbalance during train and val was overcome by the classifier.

